Laser-annealing Josephson junctions for yielding scaled-up superconducting quantum processors

As superconducting quantum circuits scale to larger sizes, the problem of frequency crowding proves a formidable task. Here we present a solution for this problem in fixed-frequency qubit architectures. By systematically adjusting qubit frequencies post-fabrication, we show a nearly ten-fold improvement in the precision of setting qubit frequencies. To assess scalability, we identify the types of 'frequency collisions' that will impair a transmon qubit and cross-resonance gate architecture. Using statistical modeling, we compute the probability of evading all such conditions, as a function of qubit frequency precision. We find that without post-fabrication tuning, the probability of finding a workable lattice quickly approaches 0. However with the demonstrated precisions it is possible to find collision-free lattices with favorable yield. These techniques and models are currently employed in available quantum systems and will be indispensable as systems continue to scale to larger sizes.

==> Resubmission to Arxiv 9-23-20 - files copied from prev submit and small edits/Yield_and_Tuning_Methods_v6c_nocomments.tex <==

%=======================================================================================
\subsection{Chip Fabrication}

A chip of the kind used to determine $\sigma_f$ and to test our laser-anneal rework process appears in \cref{fig:36Q_andTuned2f}. All microwave elements comprise Nb films $\sim$ 200 nm thick on a silicon substrate. Each qubit is coupled to a readout resonator but is not directly coupled to any nearby qubits. All transmon capacitors are identical. Junctions are fabricated using identical electron-beam lithographic patterns and deposited simultaneously using double-angle deposition and oxidation \cite{dolan_offset_1977}. The individual qubit design is similar to that used in Ref \cite{sheldon_procedure_2016} with aharmonicity $f_{12} - f_{01} \simeq $ -330 MHz. Junctions have linear dimension $\sim 100$ nm and are designed for $I_c$ of $\sim$ 30 nA. During packaging, we accidentally damaged three of the 36 qubits and found these to be non-functional when cooled in a dilution refrigerator. We left two of the remaining 33 qubits un-tuned as experimental controls, so that our tuning demonstration includes 31 qubits. \\


%=======================================================================================
\subsection{Tuning Using Selective Laser Anneal}

We have built an integrated junction rework system that can measure and modify the junction resistance. Fig. \ref{fig:LaserTuneSchematic} shows a schematic of our laser annealing system, which we call ``Laser Annealing of Stochastically Impaired Qubits'' (LASIQ). The laser output is generated by a diode-pumped solid-state laser, frequency doubled to 532 nm. Active power control of the anneal beam is performed using a piezo-rotary mounted waveplate and polarizing beam splitter (PBS), which is adaptively adjusted based on a pick-off beam measured on a downstream silicon photodiode. A precision-timed shutter is used to control the anneal duration, and beam alignment is performed using a mechanical mirror mount which directs the beam via pattern recognition to the transmon junction center. The beam is shaped as needed to avoid illuminating the junction directly \cite{rosenblatt_laser_2019-1}. \\

By careful control of laser power and pulse duration, we use this system to adjust $R_n$. This process overcomes the imprecision due to transmon fabrication, with a residual imprecision $\sigma_f$ due to the rework process. To develop the process, we prepared a set of more than 150 junctions identically to qubit junctions, and measured their response to a range of laser powers and exposure times. We recorded $R_n$ shifts up to 15\% relative to initial $R_n$, for anneal durations varying by an order of magnitude and laser powers varying by 20\%. Response to laser power in particular was highly nonlinear. Based on these empirical calibrations of $R_n$ shift to power and exposure, we established a qubit tuning process: We first measure the transmon junction's $R_n$ using four-point probing of the transmon capacitor pads at 25 \si{\degree}C. Using a $f(R_n)$ prediction based on a previously determined correlation curve (\cref{fig:36Q_andTuned2f}), we assign the junction a target resistance corresponding to the target frequency in a multiqubit chip lattice. Because the anneal can shift $R_n$ in only one direction, the target must be higher than the initial $R_n$. We anneal the qubit junction using laser power and duration chosen from our calibration set, then re-measure its $R_n$. A junction requiring large shifts in $R_n$ may require repeated anneals to reach its target, as shown in \cref{fig:LaserTuneSchematic}. The control algorithm increases the resistance until the measured value is within 0.3\% of the target value. In a separate trial of tuning precision, more than 300 junctions were tuned to target $R_n$s ranging from 0.4\% to 14.5\% above their initial values, and landed successfully within this 0.3\% margin. We expect 0.3\% imprecision in $R_n$ to introduce 0.15\% imprecision in transmon frequency.\\


%=======================================================================================
\subsection{Monte Carlo Frequency-Crowding Model}

Using a Monte Carlo model, we can estimate the incidence of `frequency collisions' in a lattice as a function of $\sigma_f$. We assume that imperfect frequency-setting will distribute qubit frequencies normally around their design frequencies with standard deviation $\sigma_f$. For lattices of the type shown in \cref{fig:lattices_and_freqs}, we designate 3 to 5 frequencies $f_1$, $f_2$, $f_3$, $f_4$, $f_5$ spaced at regular intervals in the pattern shown. We set $f_1 = 5$ GHz, similar to real-world transmons \cite{sheldon_characterizing_2016, jurcevic_demonstration_2020}. We sample the qubit frequencies randomly around these values and count the collisions throughout the lattice, as listed in \cref{table:collision_types}. This process is illustrated in \cref{fig:freqpatternexample}. We repeat the frequency-assignment and counting to build statistics for a given lattice and frequency pattern. We then repeat the model for a range of $\sigma_f$ values from 0 to 150 MHz. We repeat the entire process over a range of frequency spacings, to find the spacing that minimizes `frequency collisions' at each value of $\sigma_f$. As a function of $\sigma_f$ we can then extract 1) the mean number of total collisions in the lattice, and 2) the fraction of repetitions which result in zero collisions (`yield'). Our simulations used 1000 repetitions except to find yield below 1\% in $d = 5$ lattices and below 0.2\% in $d = 3$ lattices, which used 4000 repetitions, and in $d = 7$ lattices to find mean collisions for $\sigma_f < 16$ MHz or yield above 50\% (100 repetitions) or to find mean collisions for $\sigma_f > 16$ MHz (40 repetitions). \\ 
 
\begin{figure}
	\centerline{\includegraphics[width=9cm, trim=0.0cm 7.0cm 9.0cm 0.0cm, clip]{FrequencyPatternExample.pdf}}
	\caption{\textbf{Frequency collision statistical model.} \textbf{Left: } Square lattice, $d = 3$ with 5-frequency pattern of \cref{fig:lattices_and_freqs}: $f_1 = 5.00$, $f_2 = 5.07$, $f_3 = 5.14$, $f_4 = 5.21$, $f_5 = 5.28$ GHz. To model the lattice statistically, treat the frequencies $f_1$ to $f_5$ as means of distributions. \textbf{Right: } Mean frequencies and normal distributions characterized by $\sigma_f$. For each position in the lattice, sample from the local distribution. Choose random frequencies in this fashion, count collisions as described in \cref{table:collision_types} and repeat to gather statistical sample. Process is repeated for differing spacings between mean frequencies $f_1$ to $f_5$, and for different distribution widths $\sigma_f$.}
	\label{fig:freqpatternexample}
\end{figure}



